DELFlow: Dense Efficient Learning of Scene Flow for Large-Scale Point Clouds

Point clouds are naturally sparse, while image pixels are dense. The inconsistency limits feature fusion from both modalities for point-wise scene flow estimation. Previous methods rarely predict scene flow from the entire point clouds of the scene with one-time inference due to the memory inefficiency and heavy overhead from distance calculation and sorting involved in commonly used farthest point sampling, KNN, and ball query algorithms for local feature aggregation. To mitigate these issues in scene flow learning, we regularize raw points to a dense format by storing 3D coordinates in 2D grids. Unlike the sampling operation commonly used in existing works, the dense 2D representation 1) preserves most points in the given scene, 2) brings in a significant boost of efficiency, and 3) eliminates the density gap between points and pixels, allowing us to perform effective feature fusion. We also present a novel warping projection technique to alleviate the information loss problem resulting from the fact that multiple points could be mapped into one grid during projection when computing cost volume. Sufficient experiments demonstrate the efficiency and effectiveness of our method, outperforming the prior-arts on the FlyingThings3D and KITTI dataset.

==> tables/ablation_of_representation.tex <==
\begin{table}[!t]
  \caption{Ablation study of representation forms}
  \label{table:ablation_of_representation}
%   \vspace{-1mm}
  \centering
  \begin{tabular}{lccc}
    \toprule 
    Representation & Input point & EPE3D & EPE2D \\
    \midrule
    Sparse ($n \times 3$) & 8192 & 0.0475 & 2.5885  \\
    Dense ($H \times W \times 3$) & 56269 & \textbf{0.0388} & \textbf{2.2042} \\
    \bottomrule
  \end{tabular}
%   \vspace{-2mm}
\end{table}

==> tables/ablation_of_warping.tex <==
\begin{table}[!t]
  \caption{Ablation study of warping projection}
  \label{table:ablation_of_warping}
%   \vspace{-1mm}
  \centering
  \begin{tabular}{cccc}
    \toprule 
    Warping Projection & EPE3D & Acc3DS & Acc3DR\\
    \midrule
    \quad & 0.0418 & 0.8601 & 0.9624 \\
    $\checkmark$ & \textbf{0.0388} & \textbf{0.8739} & \textbf{0.9637}  \\
    \bottomrule
  \end{tabular}
%   \vspace{-2mm}
\end{table}

==> tables/comparison_with_sota.tex <==
\begin{table*}[htpb]
  \caption{Quantitative results compared with recent methods on FlyingThings3D dataset \cite{mayer2016large} and KITTI Scene Flow dataset \cite{menze2018object}. Quarter means training the model on one fourth of the data. Complete means using the complete dataset for training. $\uparrow$ denotes better performance with higher value, and $\downarrow$ is the opposite.}
  \label{table:res}
  \centering
  \begin{tabular}{llcccccc}
\toprule 
Dataset & Method & EPE3D $\downarrow$ & Acc3DS $\uparrow$ & Acc3DR $\uparrow$ & Outliers3D $\downarrow$ & EPE2D $\downarrow$ & Acc2D $\uparrow$\\
\midrule
\multirowcell{13}{FT3D} 
 &  ICP \cite{besl1992method}  &  0.4062 & 0.1614 & 0.3038 & 0.8796 & 23.2280 & 0.2913 \\
&  FlowNet3D \cite{liu2019flownet3d}& 0.1136 & 0.4125 & 0.7706 & 0.6016 & 5.9740 & 0.5692 \\
&  SPLATFlowNet \cite{su2018splatnet}& 0.1205 & 0.4197 & 0.7180 & 0.6187 & 6.9759 & 0.5512 \\
&  HPLFlowNet \cite{gu2019hplflownet} & 0.0696 & - & - & - & - & - \\
&  PointPWC-Net \cite{wu2019pointpwc}& 0.0588 & 0.7379 & 0.9276 & 0.3424 & 3.2390 & 0.7994 \\
&  HALFlow \cite{wang2021hierarchical} & 0.0492 & 0.7850 & 0.9468 & 0.3083 & 2.7555 & 0.8111 \\
&  FLOT \cite{puy2020flot} & 0.0520 & 0.7320 & 0.9270 & 0.3570 & - & - \\
&  HCRF-Flow \cite{li2021hcrf}& 0.0488 & 0.8337 & 0.9507 & 0.2614 & 2.5652 & 0.8704 \\
& PV-RAFT \cite{wei2021pv} & 0.0461 &0.8169 &0.9574 &0.2924 & -& -\\
&  FlowStep3D \cite{kittenplon2021flowstep3d} & 0.0455 & 0.8162 & 0.9614 & 0.2165 & - & - \\
&  Ours  & \textbf{0.0388} & \textbf{0.8739} & \textbf{0.9637} & \textbf{0.2062} & \textbf{2.2042} & \textbf{0.8762} \\
\midrule
\multirowcell{12}{KITTI} 
 & ICP \cite{besl1992method} & 0.5181 & 0.0669 & 0.1667 & 0.8712 & 27.6752 & 0.1056 \\
 & FlowNet3D \cite{liu2019flownet3d}   & 0.1767 & 0.3738 & 0.6677 & 0.5271 & 7.2141 & 0.5093 \\
 & SPLATFlowNet \cite{su2018splatnet}  & 0.1988 & 0.2174 & 0.5391 & 0.6575 & 8.2306 & 0.4189 \\
&  HPLFlowNet \cite{gu2019hplflownet}   & 0.1113 & - & - & - & - & - \\
&  PointPWC-Net \cite{wu2019pointpwc}    & 0.0694 & 0.7281 & 0.8884 & 0.2648 & 3.0062 & 0.7673 \\
& HALFlow \cite{wang2021hierarchical}    & 0.0622 & 0.7649 & 0.9026 & 0.2492 & 2.5140 & 0.8128 \\
& FLOT \cite{puy2020flot}    & 0.0560 & 0.7550 & 0.9080 & 0.2420 & - & - \\
& HCRF-Flow \cite{li2021hcrf}  & 0.0531 & \textbf{0.8631} & \textbf{0.9444} & 0.1797 & 2.0700 & 0.8656 \\
& PV-RAFT \cite{wei2021pv} & 0.0560 & 0.8226 & 0.9372 & 0.2163 & - & - \\
& FlowStep3D \cite{kittenplon2021flowstep3d}    & 0.0546 & 0.8051 & 0.9254 & \textbf{0.1492} & - & - \\
& Ours   & \textbf{0.0501} & 0.8259 & 0.9375 & 0.2225 & \textbf{1.8091} & \textbf{0.8887} \\
\bottomrule
  \end{tabular}
%   \vspace{-1mm}
\end{table*}

==> tables/kitti_result.tex <==
% \setlength{\tabcolsep}{1.5mm}
\begin{table*}[t]
	\centering
	\footnotesize
	\begin{center}
%  	\resizebox{0.7\textwidth}{!}
    {
    \begin{tabular}{lccccccccccccc}
        \toprule
        \multirow{2}{*}{\text { Method }} & \multirow{2}{*}{\text { Input }} & \multicolumn{3}{c}{\text { Disparity 1 }} & \multicolumn{3}{c}{\text { Disparity 2 }} & \multicolumn{3}{c}{\text { Optical Flow }} & \multicolumn{3}{c}{\text { Scene Flow }} \\
        & & \textit{bg} & \textit{fg} & all & \textit{bg} & \textit{fg} & all & \textit{bg} & \textit{fg} & all & \textit{bg} & \textit{fg} & all \\
        \midrule 
        OSF \cite{menze2015object} & Stereo 
        & 4.14  & 11.12  & 5.29  
        & 4.49  & 16.33  & 6.61  
        & 4.21  & 15.49  & 6.26  
        & 5.52  & 22.31  & 8.52 \\
        SSF \cite{ren2017cascaded} & Stereo 
        & 3.30  & 7.74  & 4.03  
        & 4.12  & 14.57  & 5.99  
        & 4.20  & 10.81  & 5.40  
        & 5.70  & 19.93  & 8.25 \\
        Sense \cite{jiang2019sense} & Stereo 
        & 1.91  & 2.76  & 2.05  
        & 3.43  & 5.88  & 3.87  
        & 5.90  & 6.37  & 5.98  
        & 6.71  & 10.02  & 7.30 \\
        PRSM \cite{vogel20153d} & Stereo
        & 2.93  & 10.00  & 4.10  
        & 4.13  & 12.85  & 5.69  
        & 4.33  & 10.80  & 5.50  
        & 5.54  & 17.65  & 7.71 \\
        ACOSF \cite{li2021two} & Stereo
       & 2.58  & 7.23  & 3.35  
       & 3.04  & 9.85  & 4.26  
       & 3.40  & 9.52  & 4.51  
       & 4.35  & 15.79  & 6.40 \\
        DRISF \cite{ma2019deep} & Stereo
       & 1.98  & 4.17  & 2.35  
       & 2.23  & 7.33  & 3.14  
       & 2.67  & 7.66  & 3.58  
       & 3.39  & 12.34  & 4.99 \\
        OpticalExp \cite{yang2020upgrading} & Mono + LiDAR
        & 1.34  & 3.11  & 1.63  
        & 1.89  & 6.00  & 2.62  
        & 3.50  & 5.62  & 3.89  
        & 4.24  & 9.67  & 5.21 \\
        % ISF \cite{behl2017bounding} & Stereo + LiDAR
        % & 3.74  & 5.46  & 4.02  
        % & 4.06  & 9.04  & 4.95  
        % & 4.21  & 6.83  & 4.69  
        % & 5.31  & 11.65  & 6.45 \\
        RigidMask+ISF \cite{yang2021learning} & Stereo + LiDAR
        & 1.39  & 3.30  & 1.70  
        & 1.65  & 6.20  & 2.47  
        & 2.03  & 4.85  & 2.54  
        & 2.55  & 9.15  & 3.73 \\
        RAFT-3D \cite{teed2021raft} & Mono + Depth
       & 1.34  & 3.11  & 1.63  
       & 2.00  & 5.76  & 2.67  
       & 2.69  & 5.70  & 3.23  
       & 3.48  & 9.33  & 4.53 \\
        CamLiFlow \cite{liu2022camliflow} & Mono + LiDAR 
       & 1.34  & 3.11  & 1.63  
       & 1.54  & 6.17  & 2.37  
       & 1.79  & 5.12  & 2.40  
       & 2.29  & 9.36  & 3.55 \\
        \midrule
        Ours & Mono + LiDAR 
        & \bf{1.29} & \bf{2.65} & \bf{1.51} 
        & \bf{1.54} & \bf{5.75} & \bf{2.29} 
        & 1.81 & 5.33 & 2.45 
        & \bf{2.29} & \bf{8.97} & \bf{3.49} \\
        \bottomrule
    \end{tabular}
    }
    \end{center}
    \vspace{-2mm}
    \caption{Quantitative results compared with recent methods on KITTI Scene Flow dataset \cite{menze2018object} evaluated on the non-occluded pixels. In this table, bg and fg denote the background and foreground, respectively. A lower value indicates better performance.}
  \label{table:kitti}
  \vspace{-2mm}
\end{table*}


% \setlength{\tabcolsep}{1.3mm}
% \begin{table}[t]
% 	\centering
% 	\footnotesize
% 	\begin{center}
% 		\resizebox{0.8\columnwidth}{!}
% 		{
% 			\begin{tabular}{l||cc|cc||cc}
% 			\end{tabular}
% 		}
% 	\end{center}
%     \vspace{-8pt}
% 	\caption{The LiDAR odometry results on sequences 04 and 10 of KITTI odometry dataset.}
% 	\vspace{-8pt}		
% 	\label{table:lidar4_10}
% 	\vspace{0.2cm}
% \end{table}
